Graph-controlled Permutation Mixers in QAOA for the Flexible Job-Shop Problem

One of the most promising attempts towards solving optimization problems with quantum computers in the noisy intermediate scale era of quantum computing are variational quantum algorithms. The Quantum Alternating Operator Ansatz provides an algorithmic framework for constrained, combinatorial optimization problems. As opposed to the better known standard QAOA protocol, the constraints of the optimization problem are built into the mixing layers of the ansatz circuit, thereby limiting the search to the much smaller Hilbert space of feasible solutions. In this work we develop mixing operators for a wide range of scheduling problems including the flexible job shop problem. These mixing operators are based on a special control scheme defined by a constraint graph model. After describing an explicit construction of those mixing operators, they are proven to be feasibility preserving, as well as exploring the feasible subspace.

==> Figures/FJSP_example.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{steelblue31120180}{RGB}{31,120,180}

\begin{axis}[
scaled x ticks=manual:{}{\pgfmathparse{#1}},
scaled y ticks=manual:{}{\pgfmathparse{#1}},
tick align=outside,
x grid style={darkgray176},
xmajorticks=false,
xmin=-0.735, xmax=7.735,
xtick style={color=black},
xticklabels={},
y grid style={darkgray176},
ymajorticks=false,
ymin=-0.446178239021013, ymax=1.2983203390497,
ytick style={color=black},
yticklabels={}
]
\draw[-latex,draw=black] (axis cs:0,1) -- (axis cs:1,1);
\draw[-latex,draw=black] (axis cs:0,1) -- (axis cs:0,0);
\draw[-latex,draw=black] (axis cs:0,1) -- (axis cs:1,0);
\draw[-latex,draw=black] (axis cs:1,1) -- (axis cs:0,0);
\draw[-latex,draw=black] (axis cs:1,1) -- (axis cs:1,0);
\draw[-latex,draw=black] (axis cs:0,0) -- (axis cs:1,0);
\draw[-latex,draw=black] (axis cs:3,1) -- (axis cs:4,1);
\draw[-latex,draw=black] (axis cs:3,1) -- (axis cs:3,0);
\draw[-latex,draw=black] (axis cs:3,1) -- (axis cs:4,0);
\draw[-latex,draw=black] (axis cs:4,1) -- (axis cs:3,0);
\draw[-latex,draw=black] (axis cs:4,1) -- (axis cs:4,0);
\draw[-latex,draw=black] (axis cs:3,0) -- (axis cs:4,0);
\draw[-latex,draw=black] (axis cs:6,0) -- (axis cs:7,0);
\draw[-latex,draw=black] (axis cs:0,0) -- (axis cs:3,0);
\draw[-latex,draw=black] (axis cs:0,0) -- (axis cs:4,0);
\draw[-latex,draw=black] (axis cs:1,0) -- (axis cs:3,0);
\draw[-latex,draw=black] (axis cs:1,0) -- (axis cs:4,0);
\path [draw=black]
(axis cs:0,1)
--(axis cs:3,0);

\path [draw=black]
(axis cs:0,1)
--(axis cs:4,0);

\path [draw=black]
(axis cs:1,1)
--(axis cs:3,0);

\path [draw=black]
(axis cs:1,1)
--(axis cs:4,0);

\path [draw=black]
(axis cs:0,0)
--(axis cs:3,1);

\path [draw=black]
(axis cs:0,0)
--(axis cs:4,1);

\path [draw=black]
(axis cs:1,0)
--(axis cs:3,1);

\path [draw=black]
(axis cs:1,0)
--(axis cs:4,1);

\draw[-latex,draw=black] (axis cs:3,1) -- (axis cs:0,1);
\draw[-latex,draw=black] (axis cs:4,1) -- (axis cs:0,1);
\draw[-latex,draw=black] (axis cs:3,1) -- (axis cs:1,1);
\draw[-latex,draw=black] (axis cs:4,1) -- (axis cs:1,1);
\draw[-latex,draw=black] (axis cs:3,1) -- (axis cs:0,1);
\draw[-latex,draw=black] (axis cs:4,1) -- (axis cs:1,1);
\draw[-latex,draw=black] (axis cs:0,0) -- (axis cs:3,0);
\draw[-latex,draw=black] (axis cs:0,0) -- (axis cs:6,0);
\draw[-latex,draw=black] (axis cs:1,0) -- (axis cs:4,0);
\draw[-latex,draw=black] (axis cs:1,0) -- (axis cs:7,0);
\draw[-latex,draw=black] (axis cs:3,0) -- (axis cs:6,0);
\draw[-latex,draw=black] (axis cs:4,0) -- (axis cs:7,0);
\addplot [draw=steelblue31120180, fill=steelblue31120180, mark=*, only marks]
table{%
x  y
0 1
1 1
0 0
1 0
3 1
4 1
3 0
4 0
6 0
7 0
};
\draw (axis cs:0,1) node[
  scale=0.6,
  text=black,
  rotate=0.0
]{(1, 1, 1, 1)};
\draw (axis cs:1,1) node[
  scale=0.6,
  text=black,
  rotate=0.0
]{(1, 1, 1, 2)};
\draw (axis cs:0,0) node[
  scale=0.6,
  text=black,
  rotate=0.0
]{(1, 1, 2, 1)};
\draw (axis cs:1,0) node[
  scale=0.6,
  text=black,
  rotate=0.0
]{(1, 1, 2, 2)};
\draw (axis cs:3,1) node[
  scale=0.6,
  text=black,
  rotate=0.0
]{(1, 2, 1, 1)};
\draw (axis cs:4,1) node[
  scale=0.6,
  text=black,
  rotate=0.0
]{(1, 2, 1, 2)};
\draw (axis cs:3,0) node[
  scale=0.6,
  text=black,
  rotate=0.0
]{(1, 2, 2, 1)};
\draw (axis cs:4,0) node[
  scale=0.6,
  text=black,
  rotate=0.0
]{(1, 2, 2, 2)};
\draw (axis cs:6,0) node[
  scale=0.6,
  text=black,
  rotate=0.0
]{(2, 1, 2, 1)};
\draw (axis cs:7,0) node[
  scale=0.6,
  text=black,
  rotate=0.0
]{(2, 1, 2, 2)};
\end{axis}

\end{tikzpicture}


==> HICSScontent/hicss_reviews.tex <==
\section{Reviews}
Color coding: Grün(olivfarben) sollte ohne grössere Probleme machbar sein, gelb ist etwas schwieriger. Wenn ein Punkt abgearbeitet ist, bitte durchstreichen (\sout{text}), nicht löschen.

\begin{enumerate} 
\item \textcolor{olive}{I feel that a labelled Gant chart-type figure would be helpful for the reader to more quickly intuit the notation used. On this, the constraints and permutations used could be clearly labelled and referenced. 
\item \sout{It is mentioned that arrays $a, b, z,y, c$ store intermediate information on the computation, but specifically which information is not explicitly mentioned and must be determined by the reader. It would assist the reader to explain logically what each part of the circuit is doing and why. }
\item \sout{It is not clearly mentioned in which state these registers $a, b, z,y, c$ are initialized in until they are used in the two theorems. It seems it would be appropriate to use the letter labels in the subscript of the state rather than inside the label since they refer to groups of qubits and not the states thereof. At present it is implied that they are initialized in some non-zero states described by their label, rather than the qubits with given labels being initialized in the zero state as I think is the case.}
\item \sout{In section 3.2 where you have labeled points a-g, you should include a high-level description of what the operation is doing. For example (a) to encode the QAOA state in the auxiliary array $y$, (b) change the initialization of qubits $b$ from 0 to 1. (c) Set $a_j$ to $1$ if assignment $j$ has a conflict in $y$. Set $b_j$ to 0 if assignment $j$ is present in $y$ and there is no conflict. (d) set qubit $z$ to 1 if all bits in $b$ are $1$. Meaning every present assignment has no conflict. (e) Apply the permutation and flip qubit $c$ if qubit $z$ is in the $1$ state and qubit $c$ is in the $0$ state. }
\item \sout{Point (c) has a missing ket symbol} 
\item \sout{Qubit $c$ appears the figure as a control for the multi-cnot but not in point (d). }
\item \sout{The notation $d(j)$ is used but not defined}
\item \sout{The symmetric portion of the circuit does not appear to be dependent on the permutation $\pi$ in the figures, yet there is some reference to $\mathrm{nbhd}(\pi(j))$ in point (d). If there is no dependence on the specific permutation then the product of $B_{\pi}$ blocks will have a large number of cancellations and simplify considerably.} 
\item \sout{It is not clear to me that the uncomputation results in the $y$ array of qubits being disentangled with the $x$ array and returned to the $0$ state as claimed below Figure 3.17. Uncomputing this is important as tracing over $y$ entangled with $x$ will result in a mixed state and higher than depth-$1$ QAOA would therefore not give coherent evolution. }}
\textcolor{yellow}{
\item I would recommend the addition of an appendix section in which the action of the circuit on an input state is explicitly written, demonstrating that the uncomputation results in a disentangled pure state $B(\beta) \vert x \rangle$.
\item I would be interested to know if the authors can make any practical or theoretical assumptions about the solution quality of their approach compared to the original QAOA by Farhi et al. Can we expect a better approximation ratio/factor to the global optimum for FJSP instances when using those new permutation mixing operators in comparison to the conventional QAOA approach? It might be, since the Hilbert space is much smaller and only feasible solutions are considered, but maybe the authors can elaborate on this topic in their discussion and outlook section.}
\textcolor{olive}{
\item \sout{should we maybe give every state an index, like $\ket{x}_X\otimes \ket{0}_Y\otimes \cdots$. Capital letters in the index could be helpful to understand that e.g. in $\ket{x}_X$ the index is not dependet on the $x$.}
\item \sout{Some typos found: - Page 2; Remove space after “feasible subspace.” - Page 5; Duplicate *we* in “We assume that we an implementation…” - Page 7; Remove space after “cf. fig. 2.”}}
\textcolor{yellow}{
\item Suggested modification - Incorporate a comparison between the number of qubits utilized by the proposed method and standard QAOA in the Discussion Section. - Provide a detailed discussion on the scalability of the proposed approach, specifically considering the example presented in Figure 1. }
\end{enumerate}
